An Automated Approach for Privacy Leakage Identification in IoT Apps

This paper presents a fully automated static analysis approach and a tool, Taint-Things, for the identification of tainted flows in SmartThings IoT apps. Taint-Things accurately identifies all tainted flows reported by one of the state-of-the-art tools with at least 4 times improved performance. Our approach reports potential vulnerable tainted flows in a form of a concise security slice, where the relevant parts of the code are given with the lines affecting the sensitive information, which could provide security auditors with an effective and precise tool to pinpoint security issues in SmartThings apps under test. We also present and test ways to add precision to Taint-Things by adding extra sensitivities; we provide different approaches for flow, path and context sensitive analyses through modules that can be added to Taint-Things. We present experiments to evaluate Taint-Things by running it on a SmartThings app dataset as well as testing for precision and recall on a set generated by a mutation framework to see how much coverage is achieved without adding false positives. This shows an improvement in performance both in terms of speed up to 4 folds, as well as improving the precision avoiding false positives by providing a higher level of flow and path sensitivity analysis in comparison with one of state of the art tools.

==> Sections/Approach.tex <==
\section{An Automated Approach for Privacy Leakage
Identification in IoT Apps}\label{ch:Approach}
    
    \begin{figure}[b!]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/ApproachDiagramA.png}
    \caption{Taint-Things Diagram}
    \label{fig:Approach}
    \end{figure}
    
    Focusing on the issue on privacy leakage in IoT apps, and using static analysis, we propose the following approach in our study. Using TXL, we can write a tool to analyze the source code of a groovy app directly for potential tainted flows. We can then use the tool as a core module where we can add different sensitivities to to improve the precision by enabling it to handle certain patterns better and avoid possible false positives.

    \subsection{Core module approach}
    
    In figure \ref{fig:Approach} we show the basic structure of Taint-Things. It takes a groovy source code and grammar files as input and outputs the report of whether the app is benign or does it have a tainted flow. In the case there is a tainted flow, it reports the  detected tainted flow line numbers, the marked sources and sinks along with the source code. This  is done by running it through the TXL program which is made of two parts, the abstract syntax tree generation and the flow detection.
    
    The first step is done as soon as the source code is run through TXL. Using the provided grammar TXL will parse the inputted text according to Groovy's syntax. If it fails to parse at this step it terminates and gives an error.
    
    The TXL transformation rules do the next parts. The transformation rules furthermore can be dissected into three main parts: 
    % \begin{itemize}
    %     \item The sink identification
    %     \item Backward tracing
    %     \item Data flow reporting
    % \end{itemize}

    In the first step, it marks potential leakage points, called sinks, through the program. It then backtracks from them, following variables that gets passed till it reaches the sinks. Finally, it draws the flow of the variable and checks if they contain sensitive information. If it does, it reports the flow as output along the marked sinks. 
    
    \begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ApproachDiagramB.png}
    \caption{Taint-Things with SSA form or function cloning}
    \label{fig:ApproachB}
    \end{figure}
    
    \begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ApproachDiagramC.png}
    \caption{Taint-Things with path sensitivity}
    \label{fig:ApproachC}
    \end{figure}
    
   \subsection{Enhanced approach with plugins for improving precision}

    Optionally, we can think of Taint-Things as a main core module and add plugins for added precision. Flow and context sensitivities can be added by transforming the source code into Single Statement Assignment (SSA) form or adding function clones before running it through Taint-Things as shown in listing \ref{fig:ApproachB}.  Or we can run the program through a python or a batch script to run on multiple apps at once, an approach that can be utilized in adding path sensitivity by generating multiple paths from the source code and running them in Taint-Things as shown in listing \ref{fig:ApproachC}. The following chapters will explain the details of the core module and the plugins.
    
    

==> Sections/Context.tex <==
 \section{Adding Context Sensitivity}\label{ch:Context}
 
  The previous two chapters looked into how the flow can affected through variable reassignment and how conditionals can affect that. But sometimes variable reassignment is done through a method calls. Handling method calls and their return values with precision can also pose a challenge. In this chapter we look into this case where the flow goes through method calls and how to handle the context of each call. 
  
  \subsection{Implementation}    
  A context sensitive analysis takes the context of each method call in consideration while a context insensitive approach might confuse them and mark every call to a method as tainted if at one point there were one tainted call. If we take listing \ref{list:contextSensEx} where a method gets called twice, once with a tainted flow passing through it and another with a benign flow. In a context insensitive analysis, both calls on lines 4 and 5 might be conflated; the method is marked tainted after \textit{firstCall}, so \textit{secondCall} will also be considered tainted and the flow tainted. A context sensitive approach on the other hand, doesn't confuse method calls and distinguishes each call site, so it won't mark the flow to \textit{sendSms} tainted. 
    
  \begin{lstlisting}[style=Groovy, float, floatplacement=H, linewidth= 0.9\textwidth, caption={Context Sensitivity Example },label=list:contextSensAddedEx ]
  //$sensitiveData defined
  def takeAction() {
      def message = "This contains $sensitiveData";
      def firstCall = returnMessage(message);
      def secondCall = returnMessage("no sensitive data");
      sendSms(secondCall);
  }

  private returnMessage(message) {
      return message;
  }
  \end{lstlisting}
  One way to add the sensitivity is through method cloning. Where, similar to the SSA approach, we assign each method call a unique call name and clone the function with it. This assures that each call sight is treated uniquely and no conflation happens. This can be costly if there is a lot of nesting in the methods and won't work properly in the case of recursive functions. Another disadvantage of this approach is that it affects the line numbering of the data flow; depending on where the cloned functions are placed in the source code, the data flow will go through them rather than the original methods. If we apply that to the previous listing, the result will be like listing \ref{list:contextSensAdded}.

  \begin{lstlisting}[style=Groovy, linewidth= 0.9\textwidth, caption={Function Cloning Example },label=list:contextSensAdded ]
  //$sensitiveData defined
  def takeAction() {
      def message = "This contains $sensitiveData";
      def firstCall = returnMessage1(message);
      def secondCall = returnMessage2("no sensitive data");
      sendSms(secondCall);
  }
  
  private returnMessage(message) {
      return message;
  }
  
  private returnMessage1(message) {
      return message;
  }
  
  private returnMessage2(message) {
      return message;
  }
  \end{lstlisting}
\input{Algorithms/Context}

  We wrote a TXL program that can be used to do method cloning for each method call. It starts by iterating through the program's methods, scans for any call made for them, assigns it a unique call name and clones the method using that new unique name.
  
  %Another way to achieve that would be function inlining approach, where the method call is expanded and replaced with a copy of method body instead, this process can be very costly itself and will change the structure of source code to much so we opted to avoid it.

  \subsection{Evaluation}
      
  First we wanted to make test case exemplifying context sensitivity and how it is handled by Taint-Things. Listing \ref{list:contextEvalExam} shows an example where \textit{message1} calls  \mbox{\textit{returnMehtod}} with a benign string and then gets sent through a sink. The expected result is that no tainted flow is to be reported. On SAINT, it correctly reports that there is no potential leakgage. But in Taint-Things we get a flow from the lines: 3 7 8 2 10. This shows a context insensitive behavior, where \textit{returnMehtod} got tagged as tainted because of \textit{message2}. And even though the context of  the method call in \textit{message1} is different, it still gets conflated and the flow is considered tainted because of that. But after we run the function cloning transformation on this example, Taint-Things doesn't report a tainted flow, which is the correct context-sensitive behaviour.
  
  \begin{lstlisting}[style=Groovy, float, floatplacement=H, linewidth= 0.9\textwidth, caption={Context Sensitivity Example },label=list:contextEvalExam ]
  def initialize () {
    message1 = returnMethod ("benign") 
    message2 = returnMethod ("$sensitiveData")
    sendSms (message1)
  }

  def returnMethod (x) {
    return x 
  }
  \end{lstlisting}
  
  We've also ran a test on the dataset to see how it affects the results. Like the previous comparisons, it didn't have a big difference on the dataset in terms of labeling apps as tainted or benign, thus showing that there were no false positives done due to context sensitivity in the dataset. We found that there were changes done on how many unique flows and sinks were detected as well as changes on the line numbers reported from the original source code. This is due to the flow running through the multiple newly made clone methods. Performance wise, the process of function cloning isn't heavy in itself, but as the program gets bigger and with more nested function calls, analyzing the results can be more costly.

 \input{"Tables/DetailedCloningResults"}      
 
 \subsection{Summary} In this chapter, we discussed one way to extend our approach to provide context sensitivity analysis. We used function cloning to avoid the case of method call conflation. It does change the structure of the original app and introduces new flows, which can be a disadvantage and makes proper evaluation harder.

==> Sections/Flow.tex <==
\section {Adding Flow Sensitivity}\label{ch:Flow}
  While we've seen that the core module of Taint-Thing by itself is satisfactory in terms of detecting potential leakages as the tests on the dataset show, we wanted to see if there are ways to improve it by making it more resistant to potential false positives and more precise. Since it is fast and light in its performance, in this and the following chapters, we want to explore how we can improve the precision by adding analyses sensitivities. This can help us minimize false-positives in certain cases. In this chapter we'll look into the case of flow sensitivity which is relevant in the case of variable reassignment throughout the code. 
  \begin{figure}[b!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ApproachDiagramB.png}
    \caption{Taint-Things with SSA}
    \label{fig:ApproachB2}
    \end{figure}
  \subsection{Implementation}    
  A flow sensitive analysis takes in consideration the order of statement execution in the program as well as content change in variables. A flow sensitive analysis takes the variable's value changes into consideration while an insensitive approach does not. This can result into false positive reports. Currently, this is the case with both Taint-Things and SAINT, if we test the program in listing \ref{list:flowSensEx2} they both mark the flow as malicious even though it is benign. 
  
  \begin{lstlisting}[style=Groovy, float, floatplacement=H, caption={Flow Sensitivity Example}, label=list:flowSensEx2]
    // $sensitiveData defined
    def message = "This contains $sensitiveData";
    sendPush(message);
    message = "no sensitive data"; 
    sendSms(message);
    \end{lstlisting}
  To avoid conflation in this case and achieve flow sensitivity, we can deal with each variable change as if it were a new variable; each variable would only be assigned a value once. This is the same concept used in static single assignment (SSA) form where each variable in the code is assigned a value once. Listing \ref{list:SSAex1} shows Listing \ref{list:flowSensEx2} in SSA form. We can process the inputted program and transform it into this form, which we later can chain into Taint-Things. This form will provide more precision when dealing with variable reassignments and will solve the issue of false positives resulting from them. 
  
  \begin{lstlisting}[style=Groovy, caption={SSA form Example }, label=list:SSAex1]
  // $sensitiveData defined
  def message1 = "This contains $sensitiveData";
  message2 = "no sensitive data"; 
  sendSms(message2);
  \end{lstlisting}
  
  We have implemented this approach and written a TXL program that does this transformation. Using the groovy grammar, we analyse and detect all the assignment statements in a program as well as the identifiers. Listing \ref{list:assignemtInFSE} shows the detected assignment statements in Listing \ref{list:flowSensEx2}.
  
  \begin{lstlisting}[style=Groovy, float, floatplacement=H, caption={Assignment Statements }, label=list:assignemtInFSE]
  // $sensitiveData defined
  *def message = "This contains $sensitiveData";*
  *message = "no sensitive data"*
  sendSms(message);
  \end{lstlisting}
\input{Algorithms/SSA}     

  Algorithm \ref{algo:SSA} represents this process. Starting from top to bottom. We lookup identifiers that match the one defined in the assignment statement, then we give that identifier set a new unique variable name. Repeating this processes, we go through each assignment statement and its associated identifiers. The result will be a program in SSA form, where every assignment statement gives us a uniquely named variable and avoids conflation in the case of reassignment. This can later be chained with our analysis tool, giving us a more precises analysis. 
   \input{"Tables/SSA Test Results"}
  
  Going through the program's statements, if we encounter an assignment statement, we extract the variable \textit{V} from the left-hand side (LHS). We assign a counter \textit{C(V)} for it and use that to assign a new unique variable name for it. We then go through the rest of statements and if we find a statement containing the original variable, we replace it with the new variable. After that loop is finished, we go to the next assignment statement, and if it contained the same variable name, it will increment its counter, otherwise it'll be assigned a new counter.

  \subsection{Evaluation}
  To evaluate the results of our implementation, we compared the results of our tool with and without the application of SSA. We used the previous dataset, which includes 260 IoT apps gathered from different sources. For the sake of consistency we have excluded programs that gave errors in the final results; this included 4 programs without SSA, and another 4 when adding due to the SSA TXL transformation failing on some apps. As well as 35 apps using SAINT web app at the time of the dataset collection. Table \ref{tabl:SSAresults} shows the results of this test. The criteria is based on the previous comparison done in the previous chapter. We see that Adding SSA does not affect the final result which shows that no false positives were caused from the lack of flow sensitivity. 
  \input{"Tables/Detailed SSA Test"}

  When looking in detail at the results of our tool when adding SSA form on this dataset and comparing them to the original results, we saw that the results are identical with few exceptions. This shows us that on a real dataset, most programs do not get affected by adding flow sensitive analyses and there aren't many cases of variables reassignment in a way that changes the dataflow. We have included a detailed look at the results on the benchmark apps from the dataset in in Table \ref{tabl:SSABenchDet}. We can see that the results are identical with the exception of \textit{call\_by\_reflection\_1} where the SSA form actually helps in reducing the reported flows; in this case, without SSA a variable was being conflated with a possible source and thus flows from it were reported, while the SSA assigns the variable a unique name avoiding this mixup. 
   \input{"Tables/SSA Runtime"}

  Performance wise, this functionality creates relatively little overhead. To measure that, we compare the time Taint-Things takes to run on the dataset, once with the SSA transformation chained to it and another without it. Table \ref{tabl:SSAruntime} shows that the SSA transformation had an increase in CPU time but this translated to having no significant effect on the real time.

  To accurately measure precision and recall, we used an independently generated dataset through a mutation framework that was developed by S. Parveen \cite{Mutation}. The framework generates mutants targeting the evaluation of flow analysis by altering the statements' order in benign flows to generate leaking ones. The mutants covered multiple patterns where variable reassignment happen to make the flow tainted or benign and to be leaked in multiple sink types such as leakage through the internet, notifications and messages. To compute precision and recall we used the following two equations:   
  \[precision=\frac{True Positives}{True Positives+False Positives}\]
  \[recall=\frac{True Positives}{True Positives+False Negatives}\]

  This dataset included 526 mutants, 263 benign and 263 leaking, adding SSA makes it possible to accurately report benign apps, while without it, it will be falsely reported as leaky. On the full dataset, Taint-Things achieves 100\% recall with all the 263 leaking apps detected and 50\% precision with 263 true positives out of the 526 reported leaking apps, but when adding SSA it achieves 100\% recall and 100\% precision with 263 true positives out of the 263 apps. 
  %\input{"Tables/Detailed SSA Test"}

  Overall we can see that adding flow sensitivity though SSA is inexpensive and doesn't create an overhead. While the real dataset didn't have cases where adding flow sensitivity makes a significant effect, this functionality can still help in avoiding the false positive case where a variable can be reassigned a a benign value and cases where variables can be conflated. This can be very useful if we apply mitigation to the dataflow, where we want it to be correctly marked as benign when applied.
   \input{"Tables/SSA Mutation Results"}

  One thing to note when transforming code to SSA form is the challenge of dealing with the scope. In groovy, variables are declared global by default. To make a local variable, it uses the \textit{def} keyword and then any reference to it would be local. Also variables declared locally in a method will still be accessed by block statements in that method. This makes it hard to generalize a static-analysis approach for dealing with scopes. In our SSA TXL transformation, we put precedence on the local scope by taking the structure of the inputted program into consideration. One problematic aspect of this approach is that that some block statements, such as control flow statements can modify variables outside their scope. Flow sensitivity by itself ignores that which can result into false negatives, as it either ignores variable modification inside these blocks, or in the case of a conditional statement, it'll only deal with one branch of execution. The next chapter, path sensitivity, will deal with this problem.

  \subsection{Summary}
  We can add flow sensitivity by utilizing SSA form where each variable is only assigned once. This can help us avoid false positives in the case of a tainted variable being reassigned a new benign value. This is generally not a taxing job, performance wise. And while such case is rare in the dataset, it can still be helpful especially for mitigation.

==> Sections/Path.tex <==
\section{Adding Path Sensitivity}\label{ch:Path}
  Following the previous chapter, we look in the case where the flow goes through a conditional statement, where it branches into different paths. We introduce path sensitivity and look in how we can achieve it by taking all possible branches in consideration.
  
  \subsection{Implementation}    
  A path sensitive analysis takes the execution path in consideration. This is exemplified in how it deals with conditional statements; a path sensitive analysis would treat each conditional block as a separate path. This is important when trying to convert the program into SSA form. Figure \ref{fig:paths} showcases this where the variable sent through the second \textit{sendSms} could either be \textit{variable2} or \textit{variable3} depending on whether the if-statements is executed through the true branch or the false branch.
 
 In the previous section, the limitation of our approach when dealing with flow sensitivity. The problem is exemplified when dealing with conditional statements, such as if-statements and switch statements. In our paper we're going to focus on if-statements. These present branching in the program's execution path. A precise analysis takes these branches in consideration and provides all possible cases where a leakage can occur while avoiding false positives.
  
  In its simplest form, this problem can be represented with a single if statement. This will give us two branches; a branch when true and branch when false. To achieve that and generate these paths from an inputted program, we wrote two TXL transformations. One that removes the if statement, while preserving the new lines. And another that extracts the statements from its body.
  
  At this point, we have the base case solved, but a program could be more complex; it can contain an if-else, multiple if statements, nested if statements or a combination of these. We want to generate all the possible branches from these. To solve this problem, we can recursively generate the true and false paths from the program, removing the if-statements in the process, until we reach the base case.
  \begin{figure}[t!]
      \centering
      \includegraphics[width=0.7\textwidth]{Figures/paths.png}
      \caption{Example of potential paths from an if-statement}
      \label{fig:paths}
  \end{figure}
  
  To do this, we wrote a python script. The script would be responsible for recursively calling the TXL transformation for generating the true and false paths for one if-statement at a time, taking the output and rerunning the transformations, until no if-statement is left. This way we can generate all possible paths from any program with multiple or nested if-statements. After this stage, we would have gotten all the possible paths. Figure \ref{fig:2ifpaths} shows an example of how the program would run on a program with two if statements, generated all the possible four paths. For if-else statements, for the initial implementation we were converting else statement into if-statements and generating the paths from there using the same method. This approach would end up generating four paths for an if-else statement, with two impossible paths, the path of executing both the if and else clauses and the path where neither is executed. In our later implementation, we changed the way we deal with them so that if we consider the path where the \textit{if} clause is true, the \textit{else} clause is always skipped, and if we consider the path where the \textit{if} clause is false, the textit{else} clause is always executed. This accurately produces two execution paths for the if-else statements.
  
  \begin{figure}[t!]
      \centering
      \includegraphics[width=0.5\textwidth]{Figures/path2b.png}
      \caption{Example of path generation from two if-statements}
      \label{fig:2ifpaths}
  \end{figure}
  
  As for the final output, each program would give us multiple paths. Each path would be represented by a combination of \textit{T} and \textit{F} symbols. \textit{T} for true path and \textit{F} for false. And the python script would connect these outputs with the SSA transformation and Taint-Things to preform the analysis. To give an example, if we take listing \ref{list:pathListing} as an input, the output produced by our path sensitivity framework is batch report for the two possible paths as showed in listing \ref{list:pathOutput}. We can see both possible paths generated and that one path has a tainted flow reported while the other is benign. 
  
  \begin{lstlisting}[style=Groovy, float, floatplacement=H, linewidth= 0.9\textwidth, caption={Path Sensitivity Example },label=list:pathListing ]
  //sensitiveData defined
  def test () {
    if (x) {
        message = sensitiveData 
    } else {
        message = "benign" 
    } 
    sendSms (message)
  }
  \end{lstlisting}

  \begin{lstlisting}[numbers=none, float, floatplacement=H, linewidth= 0.9\textwidth, caption={Path Sensitivity Output },label=list:pathOutput ]
  Running Test.groovy
    Path: T

        def test () {
            < 8 source > message1 = sensitiveData < / >
            < sink > sendSms (message1) < / >
        }
    
        <@\textcolor{blue}{4 8}@>
    
    Path: F
    
        def test () {
            < 8 > message2 = " benign " < / >
            < sink > sendSms (message1) < / >
        }
  \end{lstlisting}
  
 \begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ApproachDiagramC.png}
    \caption{Taint-Things with path sensitivity}
    \label{fig:ApproachB3}
    \end{figure}
  \input{Algorithms/Path}    
  
  The first thing to note is that this process can be costly in terms of performance. As we have seen, with each if-statement, the program would have double the branching. This grows exponentially with each if-statement added and eventually means that the analysis will be done 2\textsuperscript{n} the times of how many if-statements there are in the program. To illustrate the frequency of if-statements in each of the dataset's apps, in each app we counted how many if-statements exist using a TXL program, then organized the results in a histogram showing how many apps have a frequency of if-statements.  Figure \ref{fig:ifFrequency1} shows the histogram frequency of if-statements in the dataset's apps. We noted 15 apps having over 50 if-statements and can be considered outliers. We excluded these 15 apps in figure \ref{fig:ifFrequency2} to show a better detail of the frequency distribution. In our tests we've seen that a program with more than 12 if-statements becomes too large to add path sensitivity in a practical way. And since the growth is exponential, with each if-statement making at least two possible branches, we want to optimize the process and try to deal with as little if-statments as possible.
  
  One way of optimizing this is doing the transformations on all the methods at once. So, a program with two methods, each with one if-statement, would only produce two paths, instead of four. So the amount of paths generated would be the exponential of the maximum number of if-statements in one method rather than the total of if-statements in the source code. Figure \ref{fig:ifFrequency3} shows a histogram of the frequency of the maximum if-statement in one method in each app in the dataset. We can see this effectively lowering the amount of possible branches, with less apps having over 12 if-statements that we have to deal with, but this can come on the expense of context-sensitivity and sometimes ignores certain possible paths that affects a flow through multiple methods; this can happen if two methods, dependant on each other, containing if-statements that affect the same data flow.
  
  Another thing to note is that not all paths generated necessarily affect the dataflow, so some programs will have multiple paths with the same dataflows reported on different paths. One way to overcome this and provide better optimization is to only consider if-statements that affect the flow. To do that, we can perform a path-insensitive analyses to mark the sinks and backtrace, marking statements in the data flow, then performing the path sensitivity analyses where we generate paths only from if-statements containing the marked statements, and finally performing the analyses again on the paths to generate results. Adding two analysis steps is considerably cheaper than the exponential cost of performing the analyses on all if-statements that don't effect the flow. Figure \ref{fig:ifFrequency4} shows the frequency of if-statements that actually affect the flow in the apps dataset's app. It shows that it can significantly reduce the required amount of if-statements to process in most apps. 
  
  
  \begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/If-statementHistogram.png}
    \caption{If-statement frequency in the dataset apps}
    \label{fig:ifFrequency1}
  \end{figure}

  \begin{figure}[htp]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/If-statementWithoutOutliersHistogram.png}
    \caption{If-statement frequency without outlier values}
    \label{fig:ifFrequency2}
  \end{figure}
    
  \begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/If-statementInMethodsHistogram2.png}
    \caption{If-statement frequency with method-centered optimization}
    \label{fig:ifFrequency3}
  \end{figure}
  
    \begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/If-statementWithOptimizationHistogram.png}
    \caption{If-statement frequency with method-centered optimization}
    \label{fig:ifFrequency4}
  \end{figure}
  
    %\input{"Tables/Path Sensitivity Results"}
    \input{"Tables/Path Sensitivity Results Optimized"}

  \subsection{Evaluation}
  To evaluate our approach, we have run the program on the original dataset. We've gathered the results and compared them to the previous findings of our tool and SAINT's. At the first stages of our implementation, 76 apps in the dataset required more tweaks to the original grammar. This was because the path sensitivity tool was comprised of multiple TXL programs, each with its own special grammar modifications that can create conflicts and can result in the tool not working properly for some apps. In our later implementation, we refactored the tool to require minimum special grammar modification as well as less TXL programs. Table \ref{tabl:pathSenRes} shows a comparison between the results generated by Taint-Things with and without path sensitivity and SAINT. We used the optimization method described earlier, but it should be noted that there were still few apps with more than 12 if-statements that we had to skip, since they end with a large number of paths that would exceed the ability of our testing device to analyze in a practical manner. And for the sake of consistency we also skipped the apps the introduced errors just like previous comparisons.
    %\input{"Tables/Detailed Path Results"}
    \input{"Tables/Detailed Path Optimized Results"}

  Since the path tool actually generates multiple cases for each program, the criteria we followed for the classification was if at least one leaking path was detected, the program is flagged leaking as such. Table \ref{tabl:pathSenRes} shows our findings. We saw that on a real dataset, there wasn't any missmatch related to path sensitivity when it comes to determining whether a program is benign or leaking. This shows that there were no false positives related to path sensitivity on the original test. For a more detailed look in the results, we've added the detailed results on the benchmark part of the set in Table \ref{tabl:PathBenchDet} where we examine how many paths were generated and how many of them are benign, denoting a possibility of running the program in a way that doesn't leak data. We also looked how many of the leaky paths contained unique new flows, as apposed to having the same flow reporting in each of them and finally the total number of flows reported in all paths. Generally the flows reported matches the ones in the SSA form previously, but the path sensitivity gives more detail to the cases where each can happen.
  
  In the original version of the path-sensitivity approach was also independently tested on a set of mutations that were based on the original dataset to include path-sensitivity related attacks. The set included 440 mutations with different leakages of different types; through messages, posting on the internet and notifications. Our approach generated over 1480 unique flows for the mutations. When tested, it was found that our tool managed to cover all the possible flows for all the mutations, except for an estimation of 30 paths. From this set, our tool did not generate any false negatives. The results on this set showed a high level of precision and recall; the precision is 100\% since there are no false positives reported in that set, and recall is calculated as 96\%.
 
  \subsection{Summary}
  In this chapter, we discussed how path sensitivity can become a very expensive process very quickly due to the exponential growth of paths generated. And the fact that it also didn't have an affect on the real apps dataset can make its performance cost outweigh its benefit. Nonetheless we've seen ways to optimize it, by only generated paths that affect the flow, to a point where it can still be applicable on the majority of apps in the dataset. Its main benefit is to supplement flow sensitivity, taking in consideration conditionals that affect the flow and can help in certain cases to avoid false positives. It can also give an indication of the possibility of running the program without going through a tainted flow by providing which paths don't contain tainted flows or mitigates them.

==> Tables/DetailedPathResults.tex <==
\begin{table}
\begin{center}
\caption{Detailed results of path generation and analyses for the benchmarks Set}
\begin{adjustbox}{width=0.9\textwidth, keepaspectratio}
\label{tabl:PathBenchDetOld}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 & \textbf{\#Paths} & \textbf{Benign Paths} & \textbf{Leaky Paths} & \textbf{Leaky \%}  & \textbf{\#Flows}\\ \hline
\textbf{call\_by\_reflection\_1} & Error & Error & Error & Error & Error\\ \hline
\textbf{call\_by\_reflection\_2} & 16 & 16 & 0 & 0\% & 0\\ \hline
\textbf{call\_by\_reflection\_3} & 21 & 3 & 18 (7 unique) & 86\% & 9 \\ \hline
\textbf{explicit} & 21 & 3 & 18 (7 unique) & 86\% & 7\\ \hline
\textbf{global\_variable\_1} & 25 & 2 & 23 (8 unique) & 92\% & 17\\ \hline
\textbf{implicit\_1} & Error & Error & Error & Error & Error \\ \hline
\textbf{implicit\_2} & 21  & 5 & 16 (4 unique) & 76\% & 4\\ \hline
\textbf{implicit\_explicit} & 21 & 5 & 16 (5 unique) & 76\% & 7\\ \hline
\textbf{leaking\_via\_closures}  & 25  & 2 & 23 (8 unique) & 92\% & 11\\ \hline
\textbf{multiple\_devices\_1} & 25 & 5 & 20 (3 unique) & 80\% & 3\\ \hline
\textbf{multiple\_devices\_2} & 25 & 5 & 20 (2 unique) & 80\% & 4 \\ \hline
\textbf{multiple\_devices\_3} & 21 & 5 & 16 (2 unique)  & 76\% & 2\\ \hline
\textbf{multiple\_entrypoint\_1} & 21 & 5 & 16 (5 unique) & 76\% & 8\\ \hline
\textbf{multiple\_entrypoint\_2} & 21 & 2 & 19 (8 unique) & 90\% & 8\\ \hline
\textbf{multiple\_leakage\_1}    & 25 & 2 & 23 (9 unique) & 92\% & 20 \\ \hline
\textbf{multiple\_leakage\_2}    & 25 & 2 & 23 (8 unique) & 92\% & 18\\ \hline
\textbf{multiple\_leakage\_3}    & Error & Error & Error & Error & Error\\ \hline
\textbf{side\_channel\_1} & 40 & 40 & 0 & 0\% & 0\\ \hline
\textbf{side\_channel\_2} & Error & Error & Error & Error & Error\\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> Tables/Detailed_Taint-Things_and_SAINT_Old.tex <==
\begin{table}[t]
\centering
 \caption {Detailed comparison of mismatched results}
\begin{adjustbox}{width=0.7\textwidth,totalheight={0.6\textheight},keepaspectratio}%
\begin{tabular}{|l|c|c|l|}
\hline
\textbf{App Category} & \textbf{Taint-Things} & \textbf{SAINT} & \textbf{Tags}\\
\hline
\textbf{Community Mismatches}   & {}   & {}    & {}   \\
ifttt & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
hub-ip-notifier & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
%smart-auto-lock-unlock & {$\bigcirc$}   & {\xmark}    & {Tag3}   \\ gonna add this as a Leaking app wattvision-manager & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
%{} & {}   & {}    & {}\\
\textbf{Forum Mismatches}   & {}   & {}    & {}   \\
loft & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
%{} & {}   & {}    & {}\\
\textbf{Market Mismatches}  & {}   & {}    & {}   \\
curb-energy-manager & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
spruce-scheduler & {\xmark}   & {$\bigcirc$}    & {Tag2}   \\
\hline
\multicolumn{4}{l}{\footnotesize * \xmark \ denotes an app marked leaking, $\bigcirc$ denotes an app marked benign}\\
\multicolumn{4}{l}{\footnotesize * Tag 1: Unconsidered source, Tag 2: Generalizing source variables}\\
\end{tabular}
\end{adjustbox}
\label{tab1:mismatch}
\vspace{-0.6 cm}
\end{table}

==> Tables/Path_Sensitivity_Results.tex <==
\begin{table}
\caption{Path sensitivity results}
\begin{adjustbox}{width=1\textwidth, keepaspectratio}
\label{tabl:pathSenResOld}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{2}{l|}{\textbf{Taint-Things}} & \multicolumn{2}{l|}{\textbf{SSA}} & \multicolumn{2}{l|}{\textbf{Path Sensitivity}} & \multicolumn{2}{l|}{\textbf{SAINT}} \\ \hline
 & \multicolumn{1}{l|}{Benign} & \multicolumn{1}{l|}{Leaking} & \multicolumn{1}{l|}{Benign} & \multicolumn{1}{l|}{Leaking} & \multicolumn{1}{l|}{Benign} & \multicolumn{1}{l|}{Leaking} & \multicolumn{1}{l|}{Benign} & \multicolumn{1}{l|}{Leaking} \\ \hline
\textbf{Community}   & 65 & 36 & 66 & 35 & 66 & 35 & 63 & 38 \\ \hline
\textbf{Forum} & 16 & 15 & 16 & 15 & 16 & 15 & 14 & 17 \\ \hline
\textbf{Marketplace} & 11 & 16 & 11 & 16 & 11 & 16 & 11 & 16 \\ \hline
\textbf{Benchmark}   & 01 & 14 & 01 & 14 & 01 & 14 & 01 & 14 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}
